Self-supervised deep visual servoing for high precision peg-in-hole insertion

Many industrial assembly tasks involve peg-in-hole like insertions with sub-millimeter tolerances which are challenging, even in highly calibrated robot cells. Visual servoing can be employed to increase the robustness towards uncertainties in the system, however, state of the art methods either rely on accurate 3D models for synthetic renderings or manual involvement in acquisition of training data. We present a novel self-supervised visual servoing method for high precision peg-in-hole insertion, which is fully automated and does not rely on synthetic data. We demonstrate its applicability for insertion of electronic components into a printed circuit board with tight tolerances. We show that peg-in-hole insertion can be drastically sped up by preceding a robust but slow force-based insertion strategy with our proposed visual servoing method, the configuration of which is fully autonomous.

==> old_intro.tex <==
\section{Introduction}

Many industrial insertion tasks requires high precision for successful completion. When the insertion tolerances are near or lower than the accumulated uncertainties in the system, naive planning-based insertion becomes unreliable. This makes tasks which require sub-milimeter precision challenging even with careful calibration. One way to introduce robustness toward system uncertainties is through either passive or active compliance. \rlha{Jeg er ikke helt skarp på forskellen mellem compliance og robusthed. Ift. compliance under indsætningen / regulering, har jeg tænkt hvor stejl force/z kurven er. Jeg ved ikke, om compliance er det rigtige ord, men det er i hvert fald en anden slags compliance end "mekaisk robusthed", altså f.eks. at en indsætning lykkes, selvom der er et offset opga f.eks. rejfning. Rasmus fixer.}

For many industrial insertion tasks there is little passive compliance, such as the case of insertion of electronical components into a printed circuit board (PCB). Furthermore, there is no gradient information in the force feedback during attempted insertion. \rlha{man skal i hvert fald i kontkat med hullet, før der er. Rasmus fixer.} Robust insertion is therefore often achieved by an exhaustive search within the region of uncertainty around the estimated insertion point, e.g. using spiral search. While this has been shown to work for successful PCB assembly~\cite{mathiesen2021towards}, it is a slow technique if the error is significant compared to the tolerances.

Visual servoing, which is defined as a technique by which a robot is controlled through visual feedback~\cite{siciliano2009force}, relaxes the reliance on accurate calibration. Recent literature demonstrates that deep learning based visual servoing can be successfully applied to peg and hole insertion. However, the methods rely either on representative 3D models for synthetic renderings or manual involvement in the acquisition of annotated training images.

We propose that the slow but effective strategy of spiral search is used to drive self supervised learning of visual servoing for peg in hole insertions as encountered in PCB assembly. Our method is constrained to the in-plane 2D alignment of the peg perpendicular to the insertion direction, as this is the primary challenge in peg and hole insertion. In our method the error function required for visual servoing is regressed from the input of two workspace mounted cameras. A spiral search stragegy provides a method for automated aquisition of annotated training images, such that a convolutional neural network can learn to regress the in-plane euclidean error.

Our contribution is:
\begin{itemize}
    \item an in-plane deep learning based visual servoing method for submillimeter precission peg-in-hole insertion 
    \item a self supervised learning scheme based on spiral search which neither requires synthetic image generation nor manual involvement in the acquisition of training images
\end{itemize}

\begin{figure}
    \centering
    %\includegraphics[width=0.7\linewidth, trim={100, 250, 150, 350}, clip]{media/setup.jpg}
    \includegraphics[width=0.9\linewidth, trim={0, 0, 0, 0}, clip]{media/cool_img.png}
    \caption{\commentTI{Cool image}}
    \label{fig:visiontrap}
\end{figure}

The proposed method is evaluated on the insertion of \commentTI{5} different electronic components into a PCB. The evaluation shows that our proposed method enables fast and robust peg in hole insertion with sub millimeter precision.

\rlha{Jeg synes, som du lige nævnte, at man godt kan lægge lidt mere vægt på, at system-optimeringen sker automatisk}\commentTI{Gøre opmærksom på at vi afslutter med spiral search og vi bare gør det hurtigt.}

The paper is organized as follows: Section \ref{sec:related} discusses the proposed method in relation to recent literature on high precision deep visual servoing. Section \ref{sec:method} then presents the proposed method. This is followed by section \ref{sec:evaluation}, which discusses the evaluation procedure, and section \ref{sec:results}, which presents and dicusses the results of the evaluation. Finally, \ref{sec:results} presents the conclusion of the work.

%We have a system with a robot, a gripper attached to the robot, and two cameras looking towards the site, where an object should be inserted.

%When the insertion tolerances are near or lower than the accumulated uncertainties in system calibrations, grasping, etc., a naive planning-based insertion fails. 
%For many insertion problems, there is no gradient information in the force feedback, and methods thus often resolve to a slow search, like spiral search.

%Classical visual servoing relies on visual markers.
%Recent work based on learning (self-cite ftw) shows that visual servoing based on learning pre-defined keypoints on representative synthetic data can be used to obtain fast and robust insertions.
%However, they only show performance on cylindrical objects, which are easy to model synthetically, and do not propose a solution when 3D-models are not available.
